Soft X-Ray Observations of Quiescent Solar Active Regions using Novel Dual-zone Aperture X-ray Solar Spectrometer (DAXSS)

The Dual-zone Aperture X-ray Solar Spectrometer (DAXSS) was flown on 2018 June18 on the NASA 36.336 sounding rocket flight and obtained the highest resolution to date for solar soft X-ray (SXR) spectra over a broad energy range. This observation was during a time with quiescent (non-flaring) small active regions on the solar disk and when the 10.7 cm radio flux (F10.7) was 75 solar flux units (1 sfu = 10-22 W/m^2/Hz). The DAXSS instrument consists of a LASP-developed dual-zone aperture and a commercial X-ray spectrometer from Amptek that measures solar full-disk irradiance from 0.5-20 keV with a resolving power of 20 near 1 keV. This paper discusses the novel design of the spectrometer and the instrument characterization techniques. Additionally,the solar measurements obtained from the 2018 sounding rocket flight are analyzed using CHIANTI spectral models to fit the temperatures, emission measures, and relative elemental abundances of the solar corona plasma. The abundance of iron was found to be 35 percent higher than expected in the quiescent sun's corona suggesting either that our spectral models require additional sophistication or that the underlying atomic database may require updates. Future long-term systematic observations of this spectral range are needed. DAXSS will fly on the INSPIRESat-1 CubeSat in late-2020, and its SXR spectral data could provide further insight into the sources of coronal heating through modeling the changes of relative elemental abundances during developments of active regions and solar flaring events.

==> Notes_from_meeting.tex <==
- Spend more time on why getting better abundance measurements is better

- Say up front that our measurements are good for this temperature range for non-flaring 2 MK to 20 MK and for flaring sun even hotter.

- Missing SMART1, CHENDRAYAN, HINODE-ICE, CDS. make IS1 only 1 year long mission

_______________________________

 - Write up four families of temperature and emission measure fits and then create a table to publish
 
 
 -read wright2017 microflare heating solar active region
 
 -read dennis 2015 solar flare element

==> Response_to_Reviewer_Comments.tex <==
Google doc found at: \hfref{https://docs.google.com/document/d/1jWQHjucCm5ThYq1YGni_oRTH_vPmGTgH-RaPAJCBcZY/edit?usp=sharing}
